CoralStyleCLIP: Co-optimized Region and Layer Selection for Image Editing

Edit fidelity is a significant issue in open-world controllable generative image editing. Recently, CLIP-based approaches have traded off simplicity to alleviate these problems by introducing spatial attention in a handpicked layer of a StyleGAN. In this paper, we propose CoralStyleCLIP, which incorporates a multi-layer attention-guided blending strategy in the feature space of StyleGAN2 for obtaining high-fidelity edits. We propose multiple forms of our co-optimized region and layer selection strategy to demonstrate the variation of time complexity with the quality of edits over different architectural intricacies while preserving simplicity. We conduct extensive experimental analysis and benchmark our method against state-of-the-art CLIP-based methods. Our findings suggest that CoralStyleCLIP results in high-quality edits while preserving the ease of use.

==> limitations.tex <==
As also discussed in \Subsectionref{results}, CORAL based on segment selection relies on segments from a pre-trained model, which can result in over- and under-selection. An even more limiting situation arises when the driving text prompt demands significant structural changes in the image, potentially altering the segments dramatically.
